ApolloCar3D: A Large 3D Car Instance Understanding Benchmark for Autonomous Driving

Autonomous driving has attracted remarkable attention from both industry and academia. An important task is to estimate 3D properties(e.g.translation, rotation and shape) of a moving or parked vehicle on the road. This task, while critical, is still under-researched in the computer vision community - partially owing to the lack of large scale and fully-annotated 3D car database suitable for autonomous driving research. In this paper, we contribute the first large-scale database suitable for 3D car instance understanding - ApolloCar3D. The dataset contains 5,277 driving images and over 60K car instances, where each car is fitted with an industry-grade 3D CAD model with absolute model size and semantically labelled keypoints. This dataset is above 20 times larger than PASCAL3D+ and KITTI, the current state-of-the-art. To enable efficient labelling in 3D, we build a pipeline by considering 2D-3D keypoint correspondences for a single instance and 3D relationship among multiple instances. Equipped with such dataset, we build various baseline algorithms with the state-of-the-art deep convolutional neural networks. Specifically, we first segment each car with a pre-trained Mask R-CNN, and then regress towards its 3D pose and shape based on a deformable 3D car model with or without using semantic keypoints. We show that using keypoints significantly improves fitting performance. Finally, we develop a new 3D metric jointly considering 3D pose and 3D shape, allowing for comprehensive evaluation and ablation study. By comparing with human performance we suggest several future directions for further improvements.

==> related.tex <==
\section{Related works}
\label{sec:related}
Over the past decades, lots of efforts are put in 3D object understanding. Here we review the datasets and algorithms, and their relationships with our major focus on autonomous driving.

\begin{table*}[t]
\center
% \vspace{-1\baselineskip}
\renewcommand*{\arraystretch}{1.2}
\fontsize{7}{7}\selectfont
%\hspace*{-0.1cm}
\setlength\tabcolsep{1.5pt}
\begin{tabular}{lccccc}
\toprule[0.13em]
% \thickhline
Dataset & Image source  & 3D Prop. & Car keypoints  & Image $\#$ &  Cars/Image & Car $\#$  \\
\hline
\multicolumn{1}{l|}{3DObject~\cite{savarese20073d}} & Control   &   full 3D & 100  & 1     \\
\multicolumn{1}{l|}{EPFL Car~\cite{ozuysal2009pose}} & Control  &  full 3D & -  & 1    \\
\multicolumn{1}{l|}{PASCAL3D+~\cite{xiang2014beyond}} & Natural  & - & xx  &  -   \\
\multicolumn{1}{l|}{ObjectNet3D~\cite{xiang2016objectnet3d}}     & Natural & - & xx & CAD &  -   \\
\multicolumn{1}{l|}{KITTI~\cite{geiger2012we}}  & Self-driving  & 80K & xx  & -  & 3D bbox $\&$ Ori.   \\
\hline
\multicolumn{1}{l|}{ApolloCar3D}     & Self-driving & 90K & 14.3    & industry & full 3D    \\
\toprule[0.13 em]
\end{tabular}
\caption{Comparison between our data-set and existing data-set with 3D car labelling. ``full 3D'' means fitting with 3D car model.}
\end{table*}

% car key point with 3D
\paragraph{Dataset with 3D object instance}
Datasets for 3D object understanding~\cite{leibe2003analyzing,thomas2006towards,savarese20073d,moreels2007evaluation,ozuysal2009pose,lopez2010icaro} proposed in early ages are often having small scale, labelled with partial 3D properties, coarse 3D models and only containing a single object in each image. For instance, 3DObject~\cite{savarese20073d} only contains 10 instances for a car category. The EPFL Car~\cite{ozuysal2009pose} has 20 car instances with multiple viewpoints while under a clear and controlled turntable. 

To handle more realistic cases from non-controlled scenes, datasets~\cite{lim2013parsing} with nature images collected from Flickr~\cite{} platform or inside a houses~\cite{} with RGBD camera are extended for 3D object labelling with tools such as LabelMe3D~\cite{}.
The IKEA dataset~\cite{lim2013parsing} labelled few hundreds indoor images with 3D furniture models. 
PASCAL3D+~\cite{xiang2014beyond} labelled the  12 rigid categories in PASCAL VOC 2012~\cite{pascal-voc-2012} images with CAD models.
ObjectNet3D~\cite{xiang2016objectnet3d} contributes a much larger 3D object dataset with images from the ImageNet~\cite{deng2009imagenet} dataset with 100 categories. These datasets reveal the difficulties of scale and occlusion in real images, however, they are not designed for autonomous driving where images containing large amount of cars and pedestrians are required.
% In addition, the 3D CAD models fitted do not have accurate absolute object scale, yielding non-accurate distance estimation of objects in the images.
%Table 1 compares our dataset to representative datasets in the
%literature with 3D annotations. Targeting at generic object 3D pose estimation, these datasets contain 

% Compared to these datasets,
% we provide continuous viewpoint annotation to realistic images from the web.
To our best knowledge, the closest real dataset with similar goal as ours is the KITTI dataset~\cite{geiger2012we} proposed for autonomous driving, which contains ground truth depth value from LiDAR. In KITTI, each car is labelled with a 3D bounding box and corresponding orientation without 3D shape understanding, while the ones with 3D car model fitted~\cite{Menze2015ISA} for the purpose of scene flow are from only 200 images, and their car parameters are not publicly available. In our case, as shown in \figref{fig:example}, we provide fully 3D shape labelling for 90K car instances inside 5277 images with 34 man-made car 3D models with absolute size following their industry parameters, with stereo image pairs and 2D car keypoint annotations. 
%Compared to these datasets, we align a 3D shape to each 2D object and provide 3D shape
% annotation to objects, which is richer information than depth or 3D points and
%allows us to transfer meta-data from the 3D shape back to the image. 
Last, we list those key properties by comparing our data and other SOTA 3D object instance datasets in \tabref{tab:dataset}.


\paragraph{3D object instance recovery}
Commonly, recovery 3D shape of an object are from multiple frames or 3D point clouds with geometry~\cite{} or learning-based methods~\cite{Yu_2018_CVPR,Reddy_2018_CVPR}. 
% with single object
Nevertheless, addressing 3D instance understanding from a single image under non-controlled environment is ill-posed, much more challenging and attracts growing attention. With the development of deep hierarchical representation, researchers are able to achieve impressive results with supervised~\cite{fidler20123d,zia2013detailed,miao2016robust,mousavian20173d,tulsiani2015viewpoints,su2015render,xiang2015data,zia2015towards,chen2016monocular,li2016deep,poirson2016fast,massa2016crafting, chabot2017deep, Yang_2018_ECCV} or weakly supervised strategies~\cite{kundu20183d,Pavlakos_2018_CVPR,kanazawa2018learning}. 
Here we summarize these methods by tasks of single or multiple objects and granularity-level of recovered 3D models. Some works consider partial 3D representations with 3D bounding boxes and orientation~\cite{fidler20123d}. While later work extend the shape representation to coarse wire-frame skeletons~\cite{}, voxel representation~\cite{} or select from a small set of exemplar models~\cite{}. 
Recently, researchers may achieve high quality results with category-specific deformable model algorithm~\cite{} or using 3D keypoints detection~\cite{} when dealing with a single instance without mutual occlusion and truncation. Works~\cite{} combine the single instance model-based representation to multiple instance cases by combining faster-rcnn~\cite{} detection, yielding impressive 3D object understanding.
However, due to lack of real supervision, these methods are relying on differential renderer~\cite{} and do render-and-compare for supervision. 
% determined by keypoints

In our case, we are interested in high quality car 3D representation for autonomous driving with supervised learning. Therefore, we select the SOTA multi-instance 3D recovery approach using deformable model, \ie 3D-RCNN~\cite{kundu20183d} without considering 3D keypoints, and approach using 3D keypoints, \ie DeepMANTA~\cite{chabot2017deep}, when 2D keypoints are available for training. In addition, we further improved the corresponding approaches by considering mask pooling, 3D object flow to model center and multiple instance relationship, yielding significant improvement over the original pipelines.

% handling multiple instance 

% handling instance with dense must
% Since we are especially interested in to evaluate and improve SOTA strategies, we follow the pipeline of 3D-RCNN, 

% Many recent works have addressed instance-level 3D 
% scene understanding, 6, 29, 38, 33, 50, 47, 56,
% 64, 35, 2, 63, 62, 12]. 
% However, most of these approaches
% [47, 50, 33, 38] only predict object orientation. When
% it comes to shape, most methods either estimate only 3D
% bounding boxes [36, 6, 12], or coarse wire-frame skeletons
% [29, 54, 63, 62], or represent shape via an exemplar
% mesh chosen from a small set of meshes [4, 56, 35, 2]. In
% contrast, we jointly learn the detailed 3D shape along with
% pose. We make use of a compact parametric shape-space
% which has much more capacity than a small set of exemplar
% meshes and can even represent articulated objects.

% with multiple object
% In our case, we try to reach the same goal with approach like 3D-RCNN~\cite{} with fine detailed 3D shape 


